BUQEYE Guide to Projection-Based Emulators in Nuclear Physics

The BUQEYE collaboration (Bayesian Uncertainty Quantification: Errors in Your EFT) presents a pedagogical introduction to projection-based, reduced-order emulators for applications in low-energy nuclear physics. The term emulator refers here to a fast surrogate model capable of reliably approximating high-fidelity models. As the general tools employed by these emulators are not yet well-known in the nuclear physics community, we discuss variational and Galerkin projection methods, emphasize the benefits of offline-online decompositions, and explore how these concepts lead to emulators for bound and scattering systems that enable fast & accurate calculations using many different model parameter sets. We also point to future extensions and applications of these emulators for nuclear physics, guided by the mature field of model (order) reduction. All examples discussed here and more are available as interactive, open-source Python code so that practitioners can readily adapt projection-based emulators for their own work.

==> buqeye_macros.tex <==
% !TEX root = EMN_Correlations_Analysis.tex

% Define \newsubcommand:
% look whether the following character is _ and, if so, it will merge the subscripts.
\makeatletter
\newcommand\newsubcommand[3]{\newcommand#1{#2\sc@sub{#3}}}
\def\sc@sub#1{\def\sc@thesub{#1}\@ifnextchar_{\sc@mergesubs}{_{\sc@thesub}}}
\def\sc@mergesubs_#1{_{\sc@thesub#1}}

\newcommand\newsupcommand[3]{\newcommand#1{#2\sc@sup{#3}}}
\def\sc@sup#1{\def\sc@thesup{#1}\@ifnextchar^{\sc@mergesups}{^{\sc@thesup}}}
\def\sc@mergesups^#1{^{\sc@thesup#1}}
\makeatother

% Bold version of mathcal
\DeclareMathAlphabet{\mathbcal}{OMS}{cmsy}{b}{n}

% Put in repeated equation to reuse equation number with a prime (Phys Rev style guide)
\newcommand{\eqrevisited}[1]{\tag{\ref*{#1}$^\prime$}}


\newcommand{\calO}{\mathcal{O}}

% Stats
\DeclareMathOperator{\MVT}{MVT}
\DeclareMathOperator{\NIG}{NIG}  % Normal inverse gamma
\DeclareMathOperator{\IG}{IG}  % Inverse gamma
\DeclareMathOperator{\ninvchisq}{N\chi^{--2}}  % Normal Inverse chi2
\DeclareMathOperator{\invchisq}{\chi^{--2}}  % Inverse chi2
\DeclareMathOperator{\E}{\mathbb{E}}
\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator*{\argmin}{argmin}
\newcommand{\kernel}{\kappa}
\newcommand{\onevec}{\boldvec{1}}
\newcommand{\identity}{\mathds{I}}
\newcommand{\cbar}{\bar c}
\newcommand{\sdth}{\cbar}
\newcommand{\sdexp}{\sigma}
\newcommand{\sdnugget}{\sigma_n}
\def\addcite#1{\textbf{\color{red}CITE[#1]}}

% \newcommand{\test}[1]{#1^\star}
% \newcommand{\testt}[1]{#1^{\star\star}}
\newcommand{\test}[1]{#1_\star}
\newcommand{\testt}[1]{#1_{\star\star}}

\newcommand{\diagnostic}{\textup{D}}
\DeclareMathOperator{\CI}{CI}
\newcommand{\DCI}{\diagnostic_{\CI}}
\newcommand{\MD}{\textup{MD}}
\newcommand{\DMD}{\diagnostic_{\MD}}
\newcommand{\DVAR}[1]{\inputvec{D}_{\textup{#1}}}
\newcommand{\DVARIT}[1]{\inputvec{D}_{#1}}

\newcommand{\entryc}[1]{\multicolumn{1}{c}{#1}}

\newcommand{\iid}{\text{i.i.d.}}
\newcommand{\Diid}{\diagnostic_{\iid}}
\newcommand{\Dv}{\diagnostic_{\rm v}}

\newcommand{\indicator}{\mathbf{1}}

% NIG prior hyperparameters
\newcommand{\hypm}{\eta}
% \newcommand{\hypv}{v}
% \newcommand{\hypa}{a}
% \newcommand{\hypb}{b}
\newcommand{\hypdisp}{V}
\newcommand{\hypdf}{\nu}
\newcommand{\hyptau}{\tau}

\newcommand{\basisfunc}{b}
\newcommand{\basis}{B}

% \newcommand{\genobstrain}{\genobsset_{\textup{train}}}
% \newcommand{\genobsvalid}{\genobsset_{\textup{val}}}
\newcommand{\ftrain}{\inputvec{f}_{\textup{train}}}
\newcommand{\fvalid}{\inputvec{f}_{\textup{val}}}

\newcommand{\genobsmean}[1]{m_{#1}}
\newcommand{\genobscorr}[1]{R_{#1}}
\newcommand{\genobsbasisfunc}[1]{\basisfunc_{#1}}
\newcommand{\genobsbasisfunctrans}[1]{\basisfunc_{#1}}  % ^\trans
\newcommand{\tildegenobsbasisfunc}[1]{\tilde\basisfunc_{#1}}
\newcommand{\genobsbasis}[1]{\basis_{#1}}

\newcommand{\tildegenobsmean}[1]{\tilde m_{#1}}
\newcommand{\tildegenobscorr}[1]{\tilde R_{#1}}

\newcommand{\discrmean}[1]{m_{\delta #1}}
\newcommand{\discrcorr}[1]{R_{\delta #1}}
\newcommand{\discrbasisfunc}[1]{\basisfunc_{\delta #1}}
\newcommand{\discrbasisfunctrans}[1]{\basisfunc_{\delta #1}}  % ^\trans
\newcommand{\discrbasis}[1]{\basis_{\delta #1}}
\newcommand{\tildediscrbasisfunc}[1]{\tilde\basisfunc_{\delta #1}}

\newcommand{\tildediscrmean}[1]{\tilde m_{\delta #1}}
\newcommand{\tildediscrcorr}[1]{\tilde R_{\delta #1}}


% Prior hyperparameters
\newcommand{\hypprior}[1]{#1_0}
% Conditional parameters
% \newcommand{\cond}[1]{{#1}_\star}
\newcommand{\cond}[1]{#1}


% general definitions
% \newcommand{\beq}{\begin{equation}}
% \newcommand{\eeq}{\end{equation}}

% \newcommand{\bseq}{\begin{subequations}}
% \newcommand{\eseq}{\end{subequations}}

% \newcommand{\ts}{\textstyle}
% \newcommand{\ds}{\displaystyle}
% \newcommand{\wt}{\widetilde}


\newcommand{\etal}{\textit{et~al.}\xspace}
\newcommand{\Msol}{\,\text{M}_{\odot}\xspace}
\newcommand{\Abinitio}{\textit{Ab~initio}\xspace}
\newcommand{\abinitio}{\textit{ab~initio}\xspace}

\newcommand{\fm}{\, \text{fm}}
\newcommand{\fmi}{\, \text{fm}^{-1}}
\newcommand{\fmis}{\, \text{fm}^{-2}}
\newcommand{\fmiq}{\, \text{fm}^{-3}}
\newcommand{\keV}{\, \text{keV}}
\newcommand{\MeV}{\, \text{MeV}}
% \newcommand{\eft}{$\chi$EFT\xspace}

% \newcommand{\la}{\langle}
% \newcommand{\ra}{\rangle}
% \newcommand{\bu}{$\bullet$\ }
% \newcommand{\adag}{a^\dagger}

%\newcommand{\NNLO}{N$^2$LO}
%\newcommand{\NNNLO}{N$^3$LO}
\newcommand{\NLO}{\ensuremath{{\rm NLO}}\xspace}
\newcommand{\NNLO}{\ensuremath{{\rm N}{}^2{\rm LO}}\xspace}
\newcommand{\NNNLO}{\ensuremath{{\rm N}{}^3{\rm LO}}\xspace}
\newcommand{\NNNNLO}{\ensuremath{{\rm N}{}^4{\rm LO}}\xspace}
\newcommand{\NNNNLOp}{\ensuremath{{\rm N}{}^4{\rm LO}+}\xspace}
\newcommand{\NkLO}[1]{\ensuremath{\mathrm{N}^{#1}\mathrm{LO}}\xspace}


\newcommand{\nc}{n_c}
\newcommand{\neff}{\ensuremath{N_{\text{eff}}}}
\newcommand{\data}{\mathcal{D}}
\newcommand{\hyperparam}{\boldsymbol{\theta}}
\newcommand{\len}{\ell}
\newcommand{\lenvec}{\boldsymbol{\ell}}
\newcommand{\lenset}{\ensuremath{L}}
\newcommand{\lenvecset}{\ensuremath{\mathbf{L}}}
\DeclareMathOperator{\GP}{\mathcal{GP}}
\DeclareMathOperator{\TP}{\mathcal{TP}}


% Emulator macros
\newcommand{\param}{\boldsymbol{\theta}}
\newcommand{\nlecs}{n_a}
\newcommand{\nbasis}{N_b}
\newcommand{\weights}{\beta}
\newcommand{\kvpweights}{\vec{\weights}_\star}
\newcommand{\lagmult}{\lambda_\star}
\newcommand{\psitrial}{\widetilde \psi}
\newcommand{\dU}{\Delta \widetilde U}
\newcommand{\genkvp}{\mathcal{L}}

% Neutron-proton and nucleon-nucleon
\newcommand{\npr}{\ensuremath{np}}
\newcommand{\NN}{\ensuremath{NN}}

\newcommand{\boldvec}[1]{\bm{#1}}
%\newcommand{\boldvec}[1]{\mathbf{#1}}

\newcommand{\ordervec}{\vec}
\newcommand{\inputdimvec}{}
\newcommand{\inputvec}{\mathbf}
\newcommand{\func}{f}
\newcommand{\funcvec}{\inputvec{\func}}
\newcommand{\meanvec}{\inputvec{m}}

\newcommand{\muth}{m_{\textup{th}}}
\newcommand{\muthset}{\mathbf{m}_{\textup{th}}}
\newcommand{\covth}{\Sigma_{\textup{th}}}
\newcommand{\covexp}{\Sigma_{\textup{exp}}}
% \newcommand{\sdexp}{\sigma_{\textup{exp}}}

% infinite matter
\newcommand{\dens}{\rho}

\newcommand{\betavec}{{\boldsymbol{\beta}}}
% \newcommand{\muvec}{\boldsymbol{\mu}}
\newcommand{\avec}{\boldvec{a}}
\newcommand{\bvec}{\boldvec{b}}
\newcommand{\cvec}{\boldvec{c}}
\newcommand{\evec}{\boldvec{e}}
\newcommand{\nvec}{\boldvec{n}}
\newcommand{\pvec}{\boldvec{p}}
\newcommand{\qvec}{\boldvec{q}}
\newcommand{\vvec}{\boldvec{v}}
\newcommand{\xvec}{\boldvec{x}}
\newcommand{\xvecd}{\boldvec{x'}} % add by myself
\newcommand{\rvec}{\boldvec{r}}
\newcommand{\Rvec}{\boldvec{R}}
\newcommand{\svec}{\boldvec{s}}
\newcommand{\yvec}{\boldvec{y}}
\newcommand{\zvec}{\boldvec{z}}
\newcommand{\muvec}{\boldvec{\mu}}
\newcommand{\sigmavec}[1]{\boldsymbol{\sigma}^{(#1)}}
\newcommand{\ellvec}{\boldvec{\ell}}
\newcommand{\mvec}{\boldvec{m}}
\newcommand{\kvec}{\boldvec{k}}
\newcommand{\kpvec}{\boldvec{k}'}
\newcommand{\kprvec}{\boldvec{k}_{R_1}'}
\newcommand{\spvec}{\boldvec{s}'}
\newcommand{\sprvec}{\boldvec{s}_{R_1}'}
\newcommand{\kppvec}{\boldvec{k}''}
\newcommand{\kpprvec}{\boldvec{k}_{R_2}''}
\newcommand{\sppvec}{\boldvec{s}''}
\newcommand{\spprvec}{\boldvec{s}_{R_2}''}
\newsubcommand{\ckvec}{\ordervec{c}}{k}
\newcommand{\ckvecsq}{\ckvec^{\,2}}

\newsubcommand{\bkvec}{\ordervec{b}}{k}
% \newcommand{\bkvecsq}{\mathbf{b}_k^{2}}
% \newcommand{\kinparvec}{\boldvec{\alpha}}
\newcommand{\kinparvec}{\inputdimvec{x}}
\newcommand{\kinparvecset}{\inputdimvec{\inputvec{x}}}



\newcommand{\kinparvecmag}{x}
% \newsubcommand{\ckvecset}{\mathbf{C}}{k}
\newsubcommand{\ckvecset}{\ordervec{\inputvec{c}}}{k}
% \newcommand{\cbarset}{\bar{C}}
\newcommand{\cset}{C}
\newcommand{\capprox}{\ensuremath{c'}}
\newcommand{\capproxxset}{\ensuremath{C'}}
\newsubcommand{\ckvecapprox}{\mathbf{c}'}{k}
\newsubcommand{\ckvecapproxset}{\mathbf{C}'}{k}
\newcommand{\bset}{B}
\newcommand{\bapprox}{\ensuremath{b'}}
\newcommand{\bapproxset}{\ensuremath{B'}}
\newsubcommand{\bkvecapprox}{\mathbf{b}'}{k}
\newsubcommand{\bkvecset}{\mathbf{B}}{k}
\newsubcommand{\bkvecapproxset}{\mathbf{B}'}{k}


\newcommand{\genobs}{y}
\newcommand{\genobsinput}{\inputdimvec{\genobs}}
\newsubcommand{\genobsvec}{\ordervec{\genobs}}{k}
\newsubcommand{\genobsvecset}{\ordervec{\inputvec{\genobs}}}{k}
\newcommand{\genobsset}{\inputvec{\genobs}}

\newcommand{\genobsexp}{\genobs_{\textup{exp}}}        % subscript or superscript?
\newcommand{\genobsexpset}{\inputvec{\genobs}_{\textup{exp}}}
% \newcommand{\genobsvecexp}{\genobsvec_{\textup{exp}}}    % {\genobsvec^{\mathrm{exp}}}  % subscript or superscript?
\newcommand{\genobsth}{\genobs_{\textup{th}}}          % subscript or superscript?
\newcommand{\genobsthset}{\inputvec{\genobs}_{\textup{th}}}


\newcommand{\qsumm}{q}
\newcommand{\qsumv}{\hat q}

\newcommand{\kord}{k}
\newcommand{\Nexp}{N_d}
\newcommand{\Qvec}{\inputvec{Q}}  % vector of expansion parameters at kinematic points

\newcommand{\lecs}{\vec{a}}
\newcommand{\LEC}{\lecs}
\newcommand{\LECk}{\LEC_k}


\newcommand{\crms}{c_{\mathrm{rms}}}  % empirical estimate of \cbar
\newcommand{\sigmaexp}{\sigma}
\newcommand{\sigmaexpvec}{\inputvec{\sigma}}
\newcommand{\covarexp}{{\Sigma}_{\mathrm{exp}}} % removed \myvec before {\Sigma}   % covariance matrix for experimental errors
\newcommand{\covarth}{{\Sigma}_{\mathrm{th}}}  % removed \myvec before {\Sigma}   % covariance matrix for theory errors
\newcommand{\covarLEC}{{\Sigma}_{\mathrm{LECs}}}
\newcommand{\covartrunc}{{\Sigma}_{k}}


\newsubcommand{\akvec}{\mathbf{a}}{k}
\newcommand{\aset}{A}
\newcommand{\aapprox}{\ensuremath{a'}}
\newcommand{\aapproxset}{\ensuremath{A'}}
\newsubcommand{\akvecapprox}{\mathbf{a}'}{k}
\newsubcommand{\akvecset}{\mathbf{A}}{k}
\newsubcommand{\akvecapproxset}{\mathbf{A}'}{k}


% \newcommand{\bi}{\begin{itemize}}
% \newcommand{\ei}{\end{itemize}}
% \newcommand{\I}{\item}
% \newcommand{\be}{\begin{enumerate}}
% \newcommand{\ee}{\end{enumerate}}
% \newcommand{\bc}{\begin{center}}
% \newcommand{\ec}{\end{center}}


\newcommand{\Covfunc}{\ensuremath{k}}
\newcommand{\Covmat}{\vb{K}}
\newcommand{\Corrmat}{\vb{R}}
\newcommand{\Covmattest}{\boldsymbol{\Sigma}}


%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%
% The \pr command
%%%%%%%%%%%%%%%%%%%

\let\Pr\undefined{}  % Remove the definition from the Physics package

% \newcommand{\pr}{\text{pr}} % Old
\DeclareMathOperator{\pr}{pr} % Good, but want to handle sizing and | spacing?
% \DeclareDocumentCommand\pr{}{\opbraces{\prob}} % Using opbraces from physics package to resize delimeters
\newcommand{\given}{\,|\,}  % Use for | in \pr
\DeclareMathOperator{\prior}{\pi}

% From https://tex.stackexchange.com/questions/187162/vertical-bar-for-absolute-value-and-conditional-expectation
% Can use automatic resizing with * or manual with [\Big] etc.
% Also can edit the spacing that | provides via innermid
% \newcommand{\prob}{\operatorname{pr}\expectarg}
% \DeclarePairedDelimiterX{\expectarg}[1]{(}{)}{%
%   \ifnum\currentgrouptype=16 \else\begingroup\fi
%   \activatebar#1
%   \ifnum\currentgrouptype=16 \else\endgroup\fi
% }

% \newcommand{\innermid}{\nonscript\;\delimsize\vert\nonscript\;}
% \newcommand{\activatebar}{%
%   \begingroup\lccode`\~=`\|
%   \lowercase{\endgroup\let~}\innermid 
%   \mathcode`|=\string"8000
% }

%%%%%%%%%%%%%%%%%%%%%%%%






% \newcommand{\cmarg}{\mathbf{c}_{\text{marg}}}
% \newcommand{\amarg}{\mathbf{a}_{\text{marg}}}
% \newcommand{\Amat}{\widehat{A}}
% \newcommand{\ares}{\mathbf{a}_{\text{res}}}
% %newcommand{\amarg}{\mathbf{a}_{\text{marg}}}
% \newcommand{\dif}{\mathrm{d}}
% \newcommand{\alphavec}{\boldsymbol{\alpha}}
% \newcommand{\fvec}{\boldsymbol{f}}
% \newcommand{\Dvec}{\boldsymbol{D}}
% \newcommand{\Covmat}{\widehat{\boldsymbol{\Sigma}}}
% \newcommand{\Modeltxt}{$\mathcal{M}\,\,$}
% \newcommand{\ED}{\mathcal{H}}
% \newcommand{\Model}{\mathcal{M}}
% \newcommand{\lhood}{\mathcal{L}}
% \newcommand{\gth}{g_{\text{th}}}
% \newcommand{\gthtwo}{g_{\text{th},2}}
% \newcommand{\hth}{h_{\text{th}}}
% \newcommand{\MchiPT}{M_{\chi \text{PT}}}
% \newcommand{\ktilde}{\tilde{k}}
% \newcommand{\Mtilde}{\widetilde{M}}
% \newcommand{\loglammu}{\log \left( \frac{\Lambda}{\mu} \right)}
% \newcommand{\mmax}{m_{max}}
% \newcommand{\fth}{f_{\text{th}}}
% \newcommand{\xmax}{x_{\text{max}}}
\newcommand{\kmax}{k_{\text{max}}}
\newcommand{\abar}{\bar{a}}
% \newcommand{\abarfix}{\abar_{\rm fix}}

%\newcommand{\cbar}{\overline{c}}
% \newcommand{\cbar}{\bar{c}}
% \newcommand{\cbarsubk}[1]{\cbar_{(#1)}}
% \newcommand{\cbark}{\cbarsubk{k}}
% \newcommand{\cbarmin}{\cbar_{<}}
% \newcommand{\cbarmax}{\cbar_{>}}

\newcommand{\lbar}{\bar{l}}
\newcommand{\Rmat}{\widehat{R}}

\newcommand{\Q}{\ensuremath{Q}}
\newcommand{\Qapprox}{\ensuremath{Q'}}
\newcommand{\Qmax}{\Q_{\rm max}}
\newcommand{\smallscale}{\ensuremath{\mathcal{Q}}}
\newcommand{\smallscaleapprox}{\ensuremath{\mathcal{Q}'}}

\newcommand{\Elab}{E_{\rm lab}}
\newcommand{\krel}{k_{\rm rel}}
\newcommand{\prel}{p_{\rm rel}}
\newcommand{\qrel}{q_{\rm rel}}
\newcommand{\kzero}{k_0}
\newcommand{\degr}{\circ}

\newcommand{\signp}{\sigma_{np}}

\newcommand{\normal}{\mathcal{N}}

% \newcommand{\atan}{\arctan}
% \newcommand{\asin}{\arcsin}


% \newcommand{\pdf}{\pr}  % {f}   % adjust this as desired.  E.g., f --> \pr
% \newcommand{\feps}{\pdf_{\epsilon}}
% \newcommand{\CH}{CH}
% \newcommand{\CHbar}{$\overline{\rm CH}$}
% \newcommand{\aSbar}{\bar{\alpha}_S}


\newcommand{\NNLOsim}{NNLO$_\text{sim}$}
\newcommand{\NNLOsep}{NNLO$_\text{sep}$}
\newcommand{\NNLOsat}{\ensuremath{\mathrm{NNLO}_{\mathrm{sat}}}}
\newcommand{\Info}{\mathcal{H}}
\newcommand{\dobs}{\tilde{d}}
\newcommand{\Htilde}{\tilde{H}}
\newcommand{\ModelT}{\text{T}}

\newcommand{\Aaug}{\matr{A}_{\textrm{aug}}}
\newcommand{\thetavec}{\bm{\theta}}
\newcommand{\dataset}[3]{\ensuremath{{\textrm #1}#2_{(#3\%)}}}
%\newcommand{\kmax}{k_{\text{max}}}

\newcommand{\Cprime}{C$'$}

% notation for matrices
%\newcommand{\matr}[1]{\mathbf{#1}} % undergraduate algebra version
\newcommand{\matr}[1]{#1}          % pure math version
%\newcommand{\matr}[1]{\bm{#1}}     % ISO complying version

\newcommand{\transpose}[1]{{#1}^{\intercal}}
\newcommand{\trans}{\intercal}


\newcommand{\ktrue}{k^{\rm true}}
\newcommand{\atrue}{a^{\rm true}}
\newcommand{\avecmin}{\hat\avec}
\newcommand{\Nd}{N_d}

\newcommand{\chiEFT}{$\chi$EFT}
\newcommand{\chisq}{\chi^2}
\newcommand{\chisqaug}{\chisq_{\textrm aug}}
\newcommand{\avecaug}{\avec_{\textrm aug}}

\newcommand{\CHtoEKM}{CH\_to\_EKM}
\newcommand{\LamchiSB}{\Lambda_{\chi {\rm SB}}}
\newcommand{\chiPT}{\chi{\rm PT}}

% \newcommand{\Data}{\ensuremath{c_0,\ldots,c_k}}
\newcommand{\Aeps}{\ensuremath{{\rm A}_{\epsilon}}}
\newcommand{\Ceps}{\ensuremath{{\rm C}_{\epsilon}}}
\newcommand{\Aepsone}{\Aeps^{(1)}}
\newcommand{\Cepsone}{\Ceps^{(1)}}
\newcommand{\Aone}{\ensuremath{{\rm A}^{(1)}}}
\newcommand{\Bone}{\ensuremath{{\rm B}^{(1)}}}
\newcommand{\Cone}{\ensuremath{{\rm C}^{(1)}}}
\newcommand{\Af}[2]{\ensuremath{{\rm A}_{#1\text{-}#2}}}
\newcommand{\Cf}[2]{\ensuremath{{\rm C}_{#1\text{-}#2}}}
\newcommand{\Afone}[2]{\Af{#1}{#2}^{(1)}}
\newcommand{\Cfone}[2]{\Cf{#1}{#2}^{(1)}}
\newcommand{\Deltakone}{\ensuremath{\Delta_k^{(1)}}}
\newcommand{\dkp}{\ensuremath{d_k^{(p)}}}
\newcommand{\sbar}{\bar{s}}
\newcommand{\sbarmin}{\sbar_{<}}
\newcommand{\sbarmax}{\sbar_{>}}
\newcommand{\ppercentt}{\ensuremath{\left(p\%\right)_{\rm t}}}

% \newcommand{\Xref}{\ensuremath{\mathcal{X}_{\text{ref}}}}
% \newcommand{\Xrefinput}{\ensuremath{\mathbcal{X}_{\text{ref}}}}
\newcommand{\genobsref}{\ensuremath{y_{\mathrm{ref}}}}
\newcommand{\genobsrefset}{\ensuremath{\inputvec{y}_{\mathrm{ref}}}}
\newcommand{\genobsrefinput}{\ensuremath{\inputdimvec{y}_{\mathrm{ref}}}}

\newcommand{\Mmatrix}[3]{M^{#1}_{{#2}\,{#3}}}
\newcommand{\CG}[6]{\langle {#1}\,{#2}\; {#3}\,{#4} | {#5}\,{#6} \rangle}
\newcommand{\sigmatot}{\sigma_{\text{tot}}}
\newcommand{\sigmaref}{\sigma_{\text {ref}}}
\newcommand{\epsbar}{\bar\varepsilon}


\newcommand{\ppercent}{(100*p)\%}

% Glockle Coefficients
\newcommand{\aG}{\ensuremath a_G}
\newcommand{\bG}{\ensuremath b_G}
\newcommand{\cG}{\ensuremath c_G}
\newcommand{\mG}{\ensuremath m_G}
\newcommand{\gG}{\ensuremath g_G}
\newcommand{\hG}{\ensuremath h_G}

% Phase notation
\newcommand{\phase}[3]{\ensuremath{\bar\delta^{#1 #3}_{#2}}}
\newcommand{\blattphase}[3]{\ensuremath{\delta^{#1 #3}_{#2}}}
\newcommand{\epsmix}[1]{\ensuremath{\bar\epsilon_{#1}}}
\newcommand{\blattepsmix}[1]{\ensuremath{\epsilon_{#1}}}
\newcommand{\gammix}[1]{\ensuremath{\bar\gamma_{#1}}}

% R on-shell
\newcommand{\Ron}[4]{R^{#1 #4}_{#2 #3}}


% Lab system / center of momentum system
\newcommand{\ls}{l.s.}
\newcommand{\cms}{c.m.}

\newcommand{\kf}{\ensuremath{k_{\scriptscriptstyle\textrm{F}}}}
\newcommand{\kfzero}{\ensuremath{k_{\scriptscriptstyle\textrm{F,0}}}}

\newcommand{\NEVC}{\ensuremath{N_{\rm EVC}}}


% Differential taken from Physics package
% Uses smart spacing for a nice look. Requires xparse.
% https://www.ctan.org/pkg/physics?lang=en

% First, the basics:
\def\diffd{\mathrm{d}}  % Upright differentials
% \def\diffd{d}  % Italic differentials

% Now add spacing:
% Derivatives
\DeclareDocumentCommand\differential{ o g d() }{ % Differential 'd'
    % o: optional n for nth differential
    % g: optional argument for readability and to control spacing
    % d: long-form as in d(cos x)
    \IfNoValueTF{#2}{
        \IfNoValueTF{#3}
            {\diffd\IfNoValueTF{#1}{}{^{#1}}}
            {\mathinner{\diffd\IfNoValueTF{#1}{}{^{#1}}\argopen(#3\argclose)}}
        }
        {\mathinner{\diffd\IfNoValueTF{#1}{}{^{#1}}#2} \IfNoValueTF{#3}{}{(#3)}}
    }
\DeclareDocumentCommand\dd{}{\differential} % Shorthand for \differential


% Path Derivative:
\newcommand{\pathd}{\mathcal{D}}  % differential symbol for path integrals

% Now add relevant spacing and options
% Inspired by differential definition from `Physics' package at
% https://www.ctan.org/tex-archive/macros/latex/contrib/physics?lang=en
\DeclareDocumentCommand\pathdifferential{ o g d() }{ % Path 'D'
    % o: optional n for nth differential
    % g: optional argument for readability and to control spacing
    % d: long-form as in d(cos x)
    \IfNoValueTF{#2}{
        \IfNoValueTF{#3}
            {\pathd\IfNoValueTF{#1}{}{^{#1}}}
            {\mathinner{\pathd\IfNoValueTF{#1}{}{^{#1}}\argopen(#3\argclose)}}
        }
        {\mathinner{\pathd\IfNoValueTF{#1}{}{^{#1}}#2} \IfNoValueTF{#3}{}{(#3)}}
    }

\DeclareDocumentCommand\DD{}{\pathdifferential} % Shorthand for \pathdifferential

% Observable notation

% \newcommand{\dsigma}{\ensuremath{\frac{\partial\sigma}{\partial\Omega}}}

% \makeatletter
% \def\dsigma{\@ifstar\@@dsigmawithstar\@dsigma}
% \def\@dsigma{\frac{\dd\sigma}{\dd\Omega}}  % \dsigma for upright frac
% \def\@@dsigmawithstar{\dd\sigma/\dd\Omega} % \dsigma* for inline frac
% \makeatother

% From physics package. Optimal braces.
% \DeclareDocumentCommand\argopen{s}{\IfBooleanTF{#1}{\mathopen{}\mathclose\bgroup}{\mathopen{}\mathclose\bgroup\left}} % Special open grouping for argument of a function
% \DeclareDocumentCommand\argclose{s}{\IfBooleanTF{#1}{\egroup}{\aftergroup\egroup\right}} % Special close grouping for argument of a function

% \DeclareDocumentCommand\braces{}{{\ifnum\z@=`}\fi\@braces}
% \DeclareDocumentCommand\@braces{ s t\big t\Big t\bigg t\Bigg m m m }
% { % General braces with automatic and manual sizing
%     \IfBooleanTF{#1}
%     {\left#6\smash{#8}\right#7\vphantom{#8}}
%     {
%         \IfBooleanTF{#2}{\bigl#6{#8}\bigr#7}{
%             \IfBooleanTF{#3}{\Bigl#6{#8}\Bigr#7}{
%                 \IfBooleanTF{#4}{\biggl#6{#8}\biggr#7}{
%                     \IfBooleanTF{#5}{\Biggl#6{#8}\Biggr#7}{\left#6{#8}\right#7}
%                 }
%             }
%         }
%     }
%     \ifnum\z@=`{\fi}
% }

% \DeclareDocumentCommand\fbraces{ s t\big t\Big t\bigg t\Bigg m m m m }
% { % Function braces with automatic and manual sizing
%     #8
%     \IfBooleanTF{#1}
%     {\argopen#6\smash{#9}\argclose#7\vphantom{#9}}
%     {
%         \IfBooleanTF{#2}{\argopen*\bigl#6{#9}\argclose*\bigr#7}{
%             \IfBooleanTF{#3}{\argopen*\Bigl#6{#9}\argclose*\Bigr#7}{
%                 \IfBooleanTF{#4}{\argopen*\biggl#6{#9}\argclose*\biggr#7}{
%                     \IfBooleanTF{#5}
%                     {\argopen*\Biggl#6{#9}\argclose*\Biggr#7}
%                     {\argopen#6{#9}\argclose#7}
%                 }
%             }
%         }
%     }
% }
% \DeclareDocumentCommand\opbraces{ m g o d() }
% {
%     \IfNoValueTF{#2}
%     {
%         \IfNoValueTF{#3}
%             {
%                 \IfNoValueTF{#4}
%                 {#1}
%                 {\fbraces{\lparen}{\rparen}{#1}{#4}}
%             }
%             {
%                 \fbraces{\lbrack}{\rbrack}{#1}{#3}
%                 \IfNoValueTF{#4}{}{(#4)}
%             }
%     }
%     {
%         \fbraces{\lbrace}{\rbrace}{#1}{#2}
%         \IfNoValueTF{#3}{}{[#3]}
%         \IfNoValueTF{#4}{}{(#4)}
%     }
% }

% \let\exponential\exp \DeclareDocumentCommand\exp{}{\opbraces{\exponential}}

